3D Alfven wave behaviour around proper and improper magnetic null points

Context: MHD waves and magnetic null points are both prevalent in many astrophysical plasmas, including the solar atmosphere. Interaction between waves and null points has been implicated as a possible mechanism for localised heating events. Aims: Here we investigate the transient behaviour of the Alfven wave about fully 3D proper and improper 3D magnetic null points. Previously, the behaviour of fast magnetoacoustic waves at null points in 3D, cold MHD was considered by Thurgood & McLaughlin (Astronomy & Astrophysics, 2012, 545, A9). Methods: We introduce an Alfven wave into the vicinity of both proper and improper null points by numerically solving the ideal, $\beta=0$ MHD equations using the LARE3D code. A magnetic fieldline and flux-based coordinate system permits the isolation of resulting wave-modes and the analysis of their interaction. Results: We find that the Alfven wave propagates throughout the region and accumulates near the fan-plane, causing current build up. For different values of null point eccentricity, the qualitative behaviour changes only by the imposition of anisotropic pulse dilation, due to the differing rates at which fieldlines diverge from the spine. For all eccentricities, we find that the fast and Alfven waves are linearly decoupled. During the driving phase, an independently propagating fast wave is nonlinearly generated due to the ponderomotive force. Subsequently, no further excitation of fast waves occurs. Conclusions: We find that the key aspects of the theory of Alfv\'en waves about 2D null points extends intuitively to the fully 3D case; i.e. the wave propagates along fieldlines and thus accumulates at predictable parts of the topology. We also highlight that unlike in the 2D case, in 3D Alfven-wave pulses are always toroidal and thus any aspects of 2D Alfven-wave-null models that are pulse-geometry specific must be reconsidered in 3D.

==> fig/jpeg2eps <==
#!/bin/sh
#
# jpeg2eps [-v] [-c] [-d] file [file [file [file ...] ] ]
# convert each JPEG file to EPS if it exists
#
#  jpeg2eps 1.00, 3rd August 2003
#  (c) Andrew Kiss 2003 <andy@rses.anu.edu.au>
#  For the latest version & usage instructions see
#  http://rses.anu.edu.au/~andy/jpeg2eps/
#
# This is a unix shell script for driving jpeg2eps.ps, a utility for 
# converting JPEG files to EPS without decompressing the JPEG data.  The 
# output EPS file will be only about 25% larger than the original JPEG, and 
# the decompression takes place in the printer (this requires a printer which 
# can handle PostScript level 2 or better).
#
# WARNING: The EPS output filename is the same as the input filename, except 
# any trailing .jpg or .jpeg is removed and .eps is appended.  If this file 
# already exists it will be OVERWRITTEN, no questions asked.
# The file "dojpeg2eps-temp.ps" will also be written to, no questions asked.
#
# This program is free software; you can redistribute it and/or
# modify it under the terms of the GNU General Public License
# as published by the Free Software Foundation; either version 2
# of the License, or any later version. In particular, any 
# distribution or modification must include this notice.
# 
# This program is distributed in the hope that it will be useful,
# but WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
# GNU General Public License for more details.
# 
# You should have received a copy of the GNU General Public License along 
# with this program; if not, write to the Free Software Foundation, Inc., 
# 59 Temple Place - Suite 330, Boston, MA 02111-1307, USA, 
# or refer to the online version at
# http://www.gnu.org/copyleft/gpl.html

# set -n # syntax checking
# set -x # debugging

# Auto-detect paths for jpeg2eps.ps and viewjpeg.ps
# ... flexible but slow.
# uses which ==> need to chmod +x jpeg2eps.ps viewjpeg.ps
	jpeg2epspath=`which jpeg2eps.ps | tail -1`
	viewjpegpath=`which viewjpeg.ps | tail -1`

# Hard-coded paths for speed (change these to suit your installation):
#	jpeg2epspath="~/bin/jpeg2eps.ps"
#	viewjpegpath="~/bin/viewjpeg.ps"

	exitcode=0
	display=0
	files=0

#	outfile="dojpeg2eps-temp$$.ps"  # unique name - includes process ID
	outfile="dojpeg2eps-temp.ps"

    if [ $# -lt 1 ]; then   # if no arguments
		exitcode=1
	else

		echo "%!PS" > $outfile
		echo "% This is a temporary file from jpeg2eps." > $outfile
		echo "($jpeg2epspath) (r) file run begin" >> $outfile
		echo "/viewjpegpath ($viewjpegpath) def" >> $outfile
		echo "/showoutput false def" >> $outfile
		echo "/verbose false def" >> $outfile
		echo "[" >> $outfile

# parse argument list

		while [ $# -ge 1 ]; do
			case $1 in
				-v)
					echo "/verbose true def" >> $outfile
					;;
				-c)
					echo "/showoutput true def" >> $outfile
					;;
				-d)
					echo "/showoutput true def" >> $outfile
					display=1
					;;
				-*)
					echo $1": invalid option"
					exitcode=1
					;;
				*)
					if [ ! -f $1 ]; then
						echo $1": file not found"
						exitcode=1
					else  
						echo "($1)" >> $outfile
						files=1
					fi
					;;
			esac
			shift   # shift argument list to look at next argument
		done

		echo "]" >> $outfile
		echo "convertjpegs" >> $outfile
		echo "end quit" >> $outfile

		if [ $files -eq "1" ]; then
			if [ $display -eq "1" ]; then
				gs -dNOSAFER -q $outfile && \rm $outfile
			else
				gs -dNOSAFER -q -dNODISPLAY -dNOPAUSE $outfile && \rm $outfile
			fi
		else
			\rm $outfile
		fi

    fi

	if [ $exitcode -ne "0" -o $files -ne "1" ]; then
		echo $0": convert JPEG files to EPS, retaining compression."
		echo "usage: jpeg2eps [-v] [-c] [-d] filename [filename ...]"
		echo "-v: verbose"
		echo "-c: check each output EPS"
		echo "-d: display each output EPS (implies -c)"
		echo "WARNING: The EPS output filename is the same as the input filename, except" 
		echo "any trailing .jpg or .jpeg is removed and .eps is appended.  If this file"
		echo "already exists it will be OVERWRITTEN, no questions asked."
		echo "The file dojpeg2eps-temp.ps will also be written to, no questions asked."
		echo "For more info see http://rses.anu.edu.au/~andy/jpeg2eps/"
	fi

exit $exitcode

